EfficientHRNet: Efficient Scaling for Lightweight High-Resolution Multi-Person Pose Estimation

There is an increasing demand for lightweight multi-person pose estimation for many emerging smart IoT applications. However, the existing algorithms tend to have large model sizes and intense computational requirements, making them ill-suited for real-time applications and deployment on resource-constrained hardware. Lightweight and real-time approaches are exceedingly rare and come at the cost of inferior accuracy. In this paper, we present EfficientHRNet, a family of lightweight multi-person human pose estimators that are able to perform in real-time on resource-constrained devices. By unifying recent advances in model scaling with high-resolution feature representations, EfficientHRNet creates highly accurate models while reducing computation enough to achieve real-time performance. The largest model is able to come within 4.4% accuracy of the current state-of-the-art, while having 1/3 the model size and 1/6 the computation, achieving 23 FPS on Nvidia Jetson Xavier. Compared to the top real-time approach, EfficientHRNet increases accuracy by 22% while achieving similar FPS with 1/3 the power. At every level, EfficientHRNet proves to be more computationally efficient than other bottom-up 2D human pose estimation approaches, while achieving highly competitive accuracy.

==> Equations/gridSearch.tex <==
\begin{equation}
\label{eq:gridSearch}
\alpha * \beta^{2} * \gamma^{2} \approx 2
\end{equation}

==> Equations/scalingUp.tex <==
\caption{\phi = 0 (no scaling)}
\begin{equation}
\label{eq:scalingUp}
\begin{split}

\alpha = 1.2^{0} = 1 \\
\beta = 1.1^{0} = 1 \\
\gamma = 1.15^{0} = 1 \\

Scaling up: \phi = 1 \\
\alpha = 1.2^{1} = 1.2 \\
\beta = 1.1^{1} = 1.1 \\
\gamma = 1.15^{1} = 1.15
\end{split}
\end{equation}

==> Equations/width_cat.tex <==
\begin{equation}
\label{eq:widthcat}
W_{cat} = W_{b_{1}} + W_{b_{2}} + W_{b_{3}} + W_{b_{4}}
\end{equation}

==> Figures/Seg_Qual.tex <==
\begin{figure*}[t]
    \begin{minipage}[t]{0.15\textwidth}
        \centering
        \subcaption{$H_0$}
        \includegraphics[width=2.6cm, height=2.15cm]{Figures/Qual_IMGs/Seg_Qual_Simple/B0.pdf}
    \end{minipage}
    \hfill
    \begin{minipage}[t]{0.15\textwidth}
        \centering
        \subcaption{$H_{-1}$}
        \includegraphics[width=2.6cm, height=2.15cm]{Figures/Qual_IMGs/Seg_Qual_Simple/B-1.pdf}
    \end{minipage}
    \hfill
    \begin{minipage}[t]{0.15\textwidth}
        \centering
        \subcaption{$H_{-2}$}
        \includegraphics[width=2.6cm, height=2.15cm]{Figures/Qual_IMGs/Seg_Qual_Simple/B-2.pdf}
    \end{minipage}  
    \hfill
    \begin{minipage}[t]{0.15\textwidth}
        \centering
        \subcaption{$H_{-3}$}
        \includegraphics[width=2.6cm, height=2.15cm]{Figures/Qual_IMGs/Seg_Qual_Simple/B-3.pdf}
    \end{minipage}
    \hfill
    \begin{minipage}[t]{0.15\textwidth}
        \centering
        \subcaption{$H_{-4}$}
        \includegraphics[width=2.6cm, height=2.15cm]{Figures/Qual_IMGs/Seg_Qual_Simple/B-4.pdf}
    \end{minipage}  
    \label{fig:1-2-3}
    \vspace{0.18cm}
    \\
    \begin{minipage}[t]{0.15\textwidth}
        \centering
        \includegraphics[width=2.6cm, height=2.15cm]{Figures/Qual_IMGs/Seg_Qual_Medium/B0.pdf}
    \end{minipage}
    \hfill
    \begin{minipage}[t]{0.15\textwidth}
        \centering
        \includegraphics[width=2.6cm, height=2.15cm]{Figures/Qual_IMGs/Seg_Qual_Medium/B-1.pdf}
    \end{minipage}
    \hfill
    \begin{minipage}[t]{0.15\textwidth}
        \centering
        \includegraphics[width=2.6cm, height=2.15cm]{Figures/Qual_IMGs/Seg_Qual_Medium/B-2.pdf}
    \end{minipage}  
    \hfill
    \begin{minipage}[t]{0.15\textwidth}
        \centering
        \includegraphics[width=2.6cm, height=2.15cm]{Figures/Qual_IMGs/Seg_Qual_Medium/B-3.pdf}
    \end{minipage}
    \hfill
    \begin{minipage}[t]{0.15\textwidth}
        \centering
        \includegraphics[width=2.6cm, height=2.15cm]{Figures/Qual_IMGs/Seg_Qual_Medium/B-4.pdf}
    \end{minipage}  
    \label{fig:1-2-32}
    \vspace{0.18cm}
    \\
    \begin{minipage}[t]{0.15\textwidth}
        \centering
        \includegraphics[width=2.6cm, height=2.15cm]{Figures/Qual_IMGs/Seg_Qual_Complex/B0.pdf}
    \end{minipage}
    \hfill
    \begin{minipage}[t]{0.15\textwidth}
        \centering
        \includegraphics[width=2.6cm, height=2.15cm]{Figures/Qual_IMGs/Seg_Qual_Complex/B-1.pdf}
    \end{minipage}
    \hfill
    \begin{minipage}[t]{0.15\textwidth}
        \centering
        \includegraphics[width=2.6cm, height=2.15cm]{Figures/Qual_IMGs/Seg_Qual_Complex/B-2.pdf}
    \end{minipage}  
    \hfill
    \begin{minipage}[t]{0.15\textwidth}
        \centering
        \includegraphics[width=2.6cm, height=2.15cm]{Figures/Qual_IMGs/Seg_Qual_Complex/B-3.pdf}
    \end{minipage}
    \hfill
    \begin{minipage}[t]{0.15\textwidth}
        \centering
        \includegraphics[width=2.6cm, height=2.15cm]{Figures/Qual_IMGs/Seg_Qual_Complex/B-4.pdf}
    \end{minipage}  
    \hfill
    \caption{Qualitative Results for EfficientHRNet segmentation models on Cityscapes test dataset. Top to bottom: Simple, Medium and Complex examples.}
    \label{fig:seg_qual}
%    \vspace{-20pt}
\end{figure*}

==> Tables/pose.tex <==
\begin{table*}[h]
    \small
    \centering
    \resizebox{0.9\linewidth}{!}{
    \begin{tabular}{c|c|c|c|c|c|c}
        Model & Input size & \# Params & FLOPS & Accuracy  &  Runtime & FPS \\
                \hline
                \hline  
            HigherHRNet & 512 & 28.6M & 47.9B & 67.1\% & 149.6ms & 6.68   \\
            Lightweight OpenPose & 512 & 10.3M & 22.8B & 43.1\%& 59.84ms& 16.71\\ 
            \hline
            $H_{0}$ & 512 & 23.3M &25.6B & 64.8\% & 62.68ms & 15.95 \\
            $H_{-1}$ & 480 & 16M & 14.2B & 59.2\% & 76.01ms & 13.15 \\
            $H_{-2}$ & 448 & 10.3M & 7.7B & 52.9\% & 56.76ms & 17.61 \\
            $H_{-3}$ & 416 & 6.9M & 4.2B & 44.8\% & 44.74ms & 22.34 \\
            $H_{-4}$ & 384 & 3.75M & 2.1B & 35.7\% & 27.15ms & 36.82 \\
    \end{tabular}
    }
    \vspace{+10pt}
    \caption{EfficientHRNet Pose Estimation Performance Evaluation}
    \label{tab:pose}
    %\vspace{-20pt}
\end{table*}

==> Tables/seg.tex <==
\begin{table*}[t]
    \centering
    %\resizebox{\linewidth}{!}{
    \begin{tabular}{c|c|c|c|c|c|c}
        Method & Backbone & Input size & \# Params & FLOPs & mIOU & FPS \\
                \hline
                \hline
            UNet++          & ResNet-101    & 512x1024  & 59.5M     & 187.1B    & 75.5\%    & -  \\
            Dilated-ResNet  & D-ResNet-101  & 512x1024  & 52.1M     & 415.4B    & 75.7\%    & - \\
            DeepLabv3       & D-ResNet-101  & 512x1024  & 58.0M     & 444.6B    & 78.5\%    & - \\
            DeepLabv3+      & D-Xception-71 & 512x1024  & 43.5M     & 361.1B    & 79.6\%    & - \\
            PSPNet          & D-ResNet-101  & 512x1024  & 65.9M     & 504.4B    & 79.9\%    & - \\
            HRNet           & HRNet-W48     & 512x1024  & 65.7M     & 173.0B    & 79.2\%    & -   \\
            HRNet v1        & HRNet-W18     & 512x1024  & 1.5M      & 7.8B      & 70.3\%    & 5.92\\ 
            HRNet v2        & HRNet-W18     & 512x1024  & 3.9M      & 18B       & 76.2\%    & 3.46\\
            \hline
            $H_{0}$         & $B_{0}$       & 512       & 24.2M     & 23.5B     & 70.7\%    & 18.13 \\
            $H_{-1}$        & $B_{-1}$      & 480       & 16.6M     & 12.9B     & 64.7\%    & 21.32 \\
            $H_{-2}$        & $B_{-2}$      & 448       & 10.7M     & 6.9B      & 60.8\%    & 28.18  \\
            $H_{-3}$        & $B_{-3}$      & 416       & 7.2M      & 3.6B      & 57.8\%    & 39.68 \\
            $H_{-4}$        & $B_{-4}$      & 384       & 3.9M      & 1.7B      & 55.5\%    & 63.33\\
             \\ 
    \end{tabular}
    %}
    %\vspace{+10pt}
    \caption{EfficientHRNet Segmentation on Cityscapes val dataset.}
    \label{tab:seg}
    \vspace{-10pt}
\end{table*}
